Learning Human-Inspired Force Strategies for Robotic Assembly

The programming of robotic assembly tasks is a key component in manufacturing and automation. Force-sensitive assembly, however, often requires reactive strategies to handle slight changes in positioning and unforeseen part jamming. Learning such strategies from human performance is a promising approach, but faces two common challenges: the handling of low part clearances which is difficult to capture from demonstrations and learning intuitive strategies offline without access to the real hardware. We address these two challenges by learning probabilistic force strategies from data that are easily acquired offline in a robot-less simulation from human demonstrations with a joystick. We combine a Long Short Term Memory (LSTM) and a Mixture Density Network (MDN) to model human-inspired behavior in such a way that the learned strategies transfer easily onto real hardware. The experiments show a UR10e robot that completes a plastic assembly with clearances of less than 100 micrometers whose strategies were solely demonstrated in simulation.

==> Phd/Literature/JabRef_databases/Phd-thesis_machine_learning_general <==
% Encoding: ISO-8859-1

@Article{Ba2016,
  author  = {Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal = {arXiv preprint arXiv:1607.06450},
  title   = {Layer normalization},
  year    = {2016},
  file    = {:home/scherzin/Documents/Phd/Literature/Papers/Layer_Normalization.pdf:PDF},
  groups  = {scherzin:2},
  url     = {https://arxiv.org/abs/1607.06450},
}

@Article{Bengio2012,
  Title                    = {Practical recommendations for gradient-based training of deep architectures},
  Author                   = {Yoshua Bengio},
  Journal                  = {CoRR},
  Year                     = {2012},
  Volume                   = {abs/1206.5533},

  Archiveprefix            = {arXiv},
  Bibsource                = {dblp computer science bibliography, https://dblp.org},
  Biburl                   = {https://dblp.org/rec/bib/journals/corr/abs-1206-5533},
  Eprint                   = {1206.5533},
  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Practical_Recommendations_for_Gradient-Based_Training_of_Deep_Architectures.pdf:PDF},
  Timestamp                = {Wed, 07 Jun 2017 14:43:16 +0200},
  Url                      = {http://arxiv.org/abs/1206.5533}
}

@Article{Clevert2015,
  author        = {Djork{-}Arn{\'{e}} Clevert and Thomas Unterthiner and Sepp Hochreiter},
  journal       = {CoRR},
  title         = {Fast and Accurate Deep Network Learning by Exponential Linear Units (ELUs)},
  year          = {2015},
  volume        = {abs/1511.07289},
  archiveprefix = {arXiv},
  bibsource     = {dblp computer science bibliography, https://dblp.org},
  biburl        = {https://dblp.org/rec/bib/journals/corr/ClevertUH15},
  eprint        = {1511.07289},
  file          = {:home/scherzin/Documents/Phd/Literature/Articles/Fast_and_Accurate_Deep_Network_Learning_by_Exponential_Linear_Units-ELUs.pdf:PDF},
  groups        = {scherzin:1},
  timestamp     = {Wed, 07 Jun 2017 14:40:17 +0200},
  url           = {http://arxiv.org/abs/1511.07289},
}

@Article{Cooijmans2016,
  author        = {Tim Cooijmans and Nicolas Ballas and C{\'{e}}sar Laurent and Aaron C. Courville},
  journal       = {CoRR},
  title         = {Recurrent Batch Normalization},
  year          = {2016},
  volume        = {abs/1603.09025},
  archiveprefix = {arXiv},
  bibsource     = {dblp computer science bibliography, https://dblp.org},
  biburl        = {https://dblp.org/rec/bib/journals/corr/CooijmansBLC16},
  eprint        = {1603.09025},
  file          = {:home/scherzin/Documents/Phd/Literature/Papers/Recurrent_Batch_Normalization.pdf:PDF},
  groups        = {scherzin:2},
  timestamp     = {Wed, 07 Jun 2017 14:43:09 +0200},
  url           = {http://arxiv.org/abs/1603.09025},
}

@Article{DeSchutter1999,
  Title                    = {Estimating first-order geometric parameters and monitoring contact transitions during force-controlled compliant motion},
  Author                   = {De Schutter, Joris and Bruyninckx, Herman and Dutr{\'e}, Stefan and De Geeter, Jan and Katupitiya, Jayantha and Demey, Sabine and Lefebvre, Tine},
  Journal                  = {The International Journal of Robotics Research},
  Year                     = {1999},
  Number                   = {12},
  Pages                    = {1161--1184},
  Volume                   = {18},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Estimating_First-Order_Geometric_Parameters_and_Monitoring_Contact_Transitions_during_Force-Controlled_Compliant_Motion.pdf:PDF},
  Publisher                = {SAGE Publications},
  Url                      = {http://journals.sagepub.com/doi/abs/10.1177/02783649922067780}
}

@Article{DeSchutter2007,
  Title                    = {Constraint-based task specification and estimation for sensor-based robot systems in the presence of geometric uncertainty},
  Author                   = {De Schutter, Joris and De Laet, Tinne and Rutgeerts, Johan and Decr{\'e}, Wilm and Smits, Ruben and Aertbeli{\"e}n, Erwin and Claes, Kasper and Bruyninckx, Herman},
  Journal                  = {The International Journal of Robotics Research},
  Year                     = {2007},
  Number                   = {5},
  Pages                    = {433--455},
  Volume                   = {26},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Constraint-Based_Task_Specification_and_Estimation_for_Sensor-Based_Robt_Systems_in_the_Presence_of_Geometric_Uncertainty.pdf:PDF},
  Publisher                = {Sage Publications Sage UK: London, England},
  Url                      = {http://journals.sagepub.com/doi/abs/10.1177/027836490707809107}
}

@Article{Debus2004,
  Title                    = {Contact state estimation using multiple model estimation and hidden markov models},
  Author                   = {Debus, Thomas J and Dupont, Pierre E and Howe, Robert D},
  Journal                  = {The International Journal of Robotics Research},
  Year                     = {2004},
  Number                   = {4-5},
  Pages                    = {399--413},
  Volume                   = {23},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Contact_State_Estimation_using_Multiple_Model_Estimation_and_Hidden_Markov_Models.pdf:PDF},
  Publisher                = {SAGE Publications},
  Url                      = {http://journals.sagepub.com/doi/abs/10.1177/0278364904042195}
}

@Article{Erhan2010,
  Title                    = {Why does unsupervised pre-training help deep learning?},
  Author                   = {Erhan, Dumitru and Bengio, Yoshua and Courville, Aaron and Manzagol, Pierre-Antoine and Vincent, Pascal and Bengio, Samy},
  Journal                  = {Journal of Machine Learning Research},
  Year                     = {2010},
  Number                   = {Feb},
  Pages                    = {625--660},
  Volume                   = {11},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Why_Does_Unsupervised_Pre-training_Help_Deep_Learning.pdf:PDF},
  Url                      = {http://www.jmlr.org/papers/v11/erhan10a.html}
}

@InProceedings{Frogner2015,
  Title                    = {Learning with a Wasserstein loss},
  Author                   = {Frogner, Charlie and Zhang, Chiyuan and Mobahi, Hossein and Araya, Mauricio and Poggio, Tomaso A},
  Booktitle                = {Advances in Neural Information Processing Systems},
  Year                     = {2015},
  Pages                    = {2053--2061},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Learning_with_a_Wasserstein_Loss.pdf:PDF},
  Url                      = {http://papers.nips.cc/paper/5679-learning-with-a-wasserstein-loss}
}

@InProceedings{Glorot2010,
  author    = {Glorot, Xavier and Bengio, Yoshua},
  booktitle = {Proceedings of the thirteenth international conference on artificial intelligence and statistics},
  title     = {Understanding the difficulty of training deep feedforward neural networks},
  year      = {2010},
  pages     = {249--256},
  file      = {:home/scherzin/Documents/Phd/Literature/Papers/Understanding_the_Difficulty_of_Training_Deep_Feedforward_Neural_Networks.pdf:PDF},
  groups    = {scherzin:1},
  url       = {http://proceedings.mlr.press/v9/glorot10a/glorot10a.pdf?hc_location=ufi},
}

@Article{Graves2013,
  Title                    = {Generating sequences with recurrent neural networks},
  Author                   = {Graves, Alex},
  Journal                  = {arXiv preprint arXiv:1308.0850},
  Year                     = {2013},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Generating_Sequences_With_Recurrent_Neural_Networks.pdf:PDF},
  Url                      = {https://arxiv.org/abs/1308.0850}
}

@InProceedings{Haidacher2003,
  Title                    = {Estimating finger contact location and object pose from contact measurements in 3d grasping},
  Author                   = {Haidacher, Steffen and Hirzinger, Gerd},
  Booktitle                = {Robotics and Automation, 2003. Proceedings. ICRA'03. IEEE International Conference on},
  Year                     = {2003},
  Organization             = {IEEE},
  Pages                    = {1805--1810},
  Volume                   = {2},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Estimating_Finger_Contact_Location_and_Object_Pose_from_Contact_Measurements_in_3-D_Grasping.pdf:PDF},
  Url                      = {http://ieeexplore.ieee.org/abstract/document/1241856/}
}

@InProceedings{He2015,
  author    = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle = {Proceedings of the IEEE international conference on computer vision},
  title     = {Delving deep into rectifiers: Surpassing human-level performance on imagenet classification},
  year      = {2015},
  pages     = {1026--1034},
  file      = {:home/scherzin/Documents/Phd/Literature/Papers/Delving_Deep_into_Rectifiers_Surpassing_Human-Level_Performance_on_imageNet_Classification.pdf:PDF},
  groups    = {scherzin:1},
  url       = {https://www.cv-foundation.org/openaccess/content_iccv_2015/html/He_Delving_Deep_into_ICCV_2015_paper.html},
}

@Article{Hochreiter1997,
  Title                    = {Long short-term memory},
  Author                   = {Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  Journal                  = {Neural computation},
  Year                     = {1997},
  Number                   = {8},
  Pages                    = {1735--1780},
  Volume                   = {9},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Long_Short-Term_Memory.pdf:PDF},
  Publisher                = {MIT Press},
  Url                      = {https://www.mitpressjournals.org/doi/abs/10.1162/neco.1997.9.8.1735}
}

@InProceedings{Hou2017,
  Title                    = {Squared earth movers distance loss for trainingdeep neural networks on orderedclasses},
  Author                   = {Hou, Le and Yu, Chen-Ping and Samaras, Dimitris},
  Booktitle                = {NIPS Workshop},
  Year                     = {2017},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Squared_Earth_Movers_Distance_Loss_for_Training_Deep_Neural_Networks_on_Ordered-Classes.pdf:PDF},
  Url                      = {http://www.chenpingyu.org/docs/squared-earth-movers.pdf}
}

@Article{Inoue2017,
  Title                    = {Deep reinforcement learning for high precision assembly tasks},
  Author                   = {Inoue, Tadanobu and De Magistris, Giovanni and Munawar, Asim and Yokoya, Tsuyoshi and Tachibana, Ryuki},
  Journal                  = {arXiv preprint arXiv:1708.04033},
  Year                     = {2017},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Deep_Reinforcement_Learning_for_High_Precision_Assembly_Tasks.pdf:PDF},
  Url                      = {https://arxiv.org/abs/1708.04033}
}

@Article{Ioffe2015,
  author  = {Ioffe, Sergey and Szegedy, Christian},
  journal = {arXiv preprint arXiv:1502.03167},
  title   = {Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  year    = {2015},
  file    = {:home/scherzin/Documents/Phd/Literature/Papers/Batch_Normalization_Accelerating_Deep_Network_Training_by_Reducing_Internal_Covariate_Shift.pdf:PDF},
  groups  = {scherzin:2},
  url     = {https://arxiv.org/abs/1502.03167},
}

@Article{Keskar2016,
  author  = {Keskar, Nitish Shirish and Mudigere, Dheevatsa and Nocedal, Jorge and Smelyanskiy, Mikhail and Tang, Ping Tak Peter},
  journal = {arXiv preprint arXiv:1609.04836},
  title   = {On large-batch training for deep learning: Generalization gap and sharp minima},
  year    = {2016},
  file    = {:home/scherzin/Documents/Phd/Literature/Papers/On_Large-Batch_Training_for_Deep_Learning_Generalization_Gap_and_Sharp_Minima.pdf:PDF},
  groups  = {scherzin:1},
  url     = {https://arxiv.org/abs/1609.04836},
}

@InProceedings{Kroeger2017,
  Title                    = {Sensor-based control, real-time motion planning, and reinforcement learning for industrial robots},
  Author                   = {T. Kroeger},
  Booktitle                = {2017 IEEE/SICE International Symposium on System Integration (SII)},
  Year                     = {2017},
  Month                    = {Dec},
  Pages                    = {3-3},

  Abstract                 = {Embedding multiple sensors - force/torque, vision, and distance - in the feedback loops of motion controllers has enabled new robot applications. For instance, safe human-robot interaction and many assembly tasks that could not be automated before. As important as these real-time control features is the ability to plan robot motions deterministically and in real-time. To enable spontaneous changes from sensor-guided robot motion control (e.g., force/torque or visual servo control) to trajectory-following motion control, an algorithmic framework is explained that lets us compute robot motions deterministically within less than one millisecond. The resulting class of on-line trajectory generation algorithms serves as an intermediate layer between low-level motion control and high-level sensor-based motion planning. Online motion generation from arbitrary states is an essential feature for autonomous hybrid switched motion control systems. Building upon this framework and with the goal of significantly reducing the amount of resources needed for programing industrial and service robots, reinforcement learning offers a yet unused potential that will be introduced as well. Samples and use-cases - including manipulation and human-robot interaction tasks - will accompany the talk in order to provide a comprehensible insight into these interesting and relevant fields of robotics.},
  Doi                      = {10.1109/SII.2017.8279182},
  File                     = {:home/scherzin/Documents/Phd/Literature/Other/Sensor-based_Control_Real-time_Motion_Planning_and_Reinforcement_Learning_for_Industrial_Robots.pdf:PDF},
  Keywords                 = {Motion control;Planning;Real-time systems;Robot motion;Robot sensing systems;Service robots}
}

@Article{Lipton2015,
  Title                    = {A critical review of recurrent neural networks for sequence learning},
  Author                   = {Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  Journal                  = {arXiv preprint arXiv:1506.00019},
  Year                     = {2015},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/A_Critical_Review_of_Recurrent_Neural_Networks_for_Sequence_Learning.pdf:PDF},
  Url                      = {https://arxiv.org/abs/1506.00019}
}

@InProceedings{Marchi2015,
  Title                    = {A novel approach for automatic acoustic novelty detection using a denoising autoencoder with bidirectional LSTM neural networks},
  Author                   = {Marchi, Erik and Vesperini, Fabio and Eyben, Florian and Squartini, Stefano and Schuller, Bj{\"o}rn},
  Booktitle                = {Acoustics, Speech and Signal Processing (ICASSP), 2015 IEEE International Conference on},
  Year                     = {2015},
  Organization             = {IEEE},
  Pages                    = {1996--2000},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/A_Novel_Approach_for_Automatic_Acoustic_Novelty_Detection_using_a_Denoising_Autoencoder_with_Bidirectional_LSTM_Neural_Networks.pdf:PDF},
  Url                      = {https://ieeexplore.ieee.org/abstract/document/7178320/}
}

@Article{Masters2018,
  author        = {Dominic Masters and Carlo Luschi},
  journal       = {CoRR},
  title         = {Revisiting Small Batch Training for Deep Neural Networks},
  year          = {2018},
  volume        = {abs/1804.07612},
  archiveprefix = {arXiv},
  bibsource     = {dblp computer science bibliography, https://dblp.org},
  biburl        = {https://dblp.org/rec/bib/journals/corr/abs-1804-07612},
  eprint        = {1804.07612},
  file          = {:home/scherzin/Documents/Phd/Literature/Articles/Revisiting_Small_Batch_Training_for_Deep_Neural_Networks.pdf:PDF},
  groups        = {scherzin:1},
  timestamp     = {Wed, 02 May 2018 15:55:01 +0200},
  url           = {http://arxiv.org/abs/1804.07612},
}

@Article{meeussen2007contact,
  Title                    = {Contact-state segmentation using particle filters for programming by human demonstration in compliant-motion tasks},
  Author                   = {Meeussen, Wim and Rutgeerts, Johan and Gadeyne, Klaas and Bruyninckx, Herman and De Schutter, Joris},
  Journal                  = {IEEE Transactions on Robotics},
  Year                     = {2007},
  Number                   = {2},
  Pages                    = {218--231},
  Volume                   = {23},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Contact_State_Segmentation_using_Particle_Filters_for_Programming_by_Human_Demonstration_in_Compliant_Motion_Tasks.pdf:PDF},
  Publisher                = {IEEE},
  Url                      = {http://ieeexplore.ieee.org/abstract/document/4154830/?reload=true}
}

@Article{Neu2012,
  Title                    = {Apprenticeship learning using inverse reinforcement learning and gradient methods},
  Author                   = {Neu, Gergely and Szepesv{\'a}ri, Csaba},
  Journal                  = {arXiv preprint arXiv:1206.5264},
  Year                     = {2012},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Apprenticeship_Learning_using_Inverse_Reinforcement_Learning_and_Gradient_Methods.pdf:PDF},
  Url                      = {https://arxiv.org/abs/1206.5264}
}

@Article{5288526,
  Title                    = {A Survey on Transfer Learning},
  Author                   = {S. J. Pan and Q. Yang},
  Journal                  = {IEEE Transactions on Knowledge and Data Engineering},
  Year                     = {2010},

  Month                    = {Oct},
  Number                   = {10},
  Pages                    = {1345-1359},
  Volume                   = {22},

  Doi                      = {10.1109/TKDE.2009.191},
  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/A_Survey_on_Transfer_Learning.pdf:PDF},
  ISSN                     = {1041-4347},
  Keywords                 = {knowledge engineering;learning by example;optimisation;unsupervised learning;machine learning;data mining;knowledge transfer;inductive transfer learning;transductive transfer learning;unsupervised transfer learning;Machine learning;Training data;Data mining;Knowledge transfer;Space technology;Knowledge engineering;Machine learning algorithms;Labeling;Learning systems;Testing;Transfer learning;survey;machine learning;data mining.}
}

@Article{Pascanu2013,
  Title                    = {How to construct deep recurrent neural networks},
  Author                   = {Pascanu, Razvan and Gulcehre, Caglar and Cho, Kyunghyun and Bengio, Yoshua},
  Journal                  = {arXiv preprint arXiv:1312.6026},
  Year                     = {2013},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/How_to_Construct_Deep_Recurrent_Neural_Networks.pdf:PDF},
  Url                      = {https://arxiv.org/pdf/1312.6026.pdf}
}

@Article{Rahmatizadeh2016,
  Title                    = {From virtual demonstration to real-world manipulation using LSTM and MDN},
  Author                   = {Rahmatizadeh, Rouhollah and Abolghasemi, Pooya and Behal, Aman and B{\"o}l{\"o}ni, Ladislau},
  Journal                  = {arXiv preprint arXiv:1603.03833},
  Year                     = {2016},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/From_Virtual_Demonstration_to_Real-World_Manipulation_Using_LSTM_and_MDN.pdf:PDF},
  Url                      = {https://arxiv.org/pdf/1603.03833.pdf}
}

@InProceedings{Sutskever2013,
  author    = {Sutskever, Ilya and Martens, James and Dahl, George and Hinton, Geoffrey},
  booktitle = {International conference on machine learning},
  title     = {On the importance of initialization and momentum in deep learning},
  year      = {2013},
  pages     = {1139--1147},
  file      = {:home/scherzin/Documents/Phd/Literature/Articles/On_The_Importance_of_Initialization_and_Momentum_in_Deep_Learning.pdf:PDF},
  groups    = {scherzin:1},
  url       = {http://proceedings.mlr.press/v28/sutskever13.pdf},
}

@InProceedings{Tang2016,
  Title                    = {Autonomous alignment of peg and hole by force/torque measurement for robotic assembly},
  Author                   = {Tang, Te and Lin, Hsien-Chung and Zhao, Yu and Chen, Wenjie and Tomizuka, Masayoshi},
  Booktitle                = {Automation Science and Engineering (CASE), 2016 IEEE International Conference on},
  Year                     = {2016},
  Organization             = {IEEE},
  Pages                    = {162--167},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Autonomous_Alignment_of_Peg_and_Hole_by_Force-Torque_Measurement_for_Robotic_Assembly.pdf:PDF},
  Url                      = {http://ieeexplore.ieee.org/abstract/document/7743375/}
}

@Article{Vincent2010,
  Title                    = {Stacked denoising autoencoders: Learning useful representations in a deep network with a local denoising criterion},
  Author                   = {Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine},
  Journal                  = {Journal of machine learning research},
  Year                     = {2010},
  Number                   = {Dec},
  Pages                    = {3371--3408},
  Volume                   = {11},

  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/Stacked_Denoising_Autoencoders_Learning_Useful_Representations_in_a_Deep_Network_with_a_Local_Denoising_Criterion.pdf:PDF},
  Url                      = {http://www.jmlr.org/papers/v11/vincent10a.html}
}

@InProceedings{Vinyals2015,
  Title                    = {Show and tell: A neural image caption generator},
  Author                   = {Vinyals, Oriol and Toshev, Alexander and Bengio, Samy and Erhan, Dumitru},
  Booktitle                = {Proceedings of the IEEE conference on computer vision and pattern recognition},
  Year                     = {2015},
  Pages                    = {3156--3164},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Show_and_Tell_A_Neural_Image_Caption_Generator.pdf:PDF},
  Url                      = {https://www.cv-foundation.org/openaccess/content_cvpr_2015/html/Vinyals_Show_and_Tell_2015_CVPR_paper.html}
}

@Article{Wang2018,
  Title                    = {MASD: A Multimodal Assembly Skill Decoding System for Robot Programming by Demonstration},
  Author                   = {Y. Wang and Y. Jiao and R. Xiong and H. Yu and J. Zhang and Y. Liu},
  Journal                  = {IEEE Transactions on Automation Science and Engineering},
  Year                     = {2018},
  Number                   = {99},
  Pages                    = {1-13},
  Volume                   = {PP},

  Abstract                 = {Programming by demonstration (PBD) transforms the robot programming from the code level to automated interface between robot and human, promoting the flexibility of robotized automation. In this paper, we focus on programming the industrial robot for assembly tasks by parsing the human demonstration into a series of assembly skills and compiling the skill to the robot executables. To achieve this goal, an identification system using multimodal information to recognize the assembly skill, called MASD, is proposed including: 1) an initial learning stage using a hierarchical model to recognize the action by considering the features from action-object effect, gesture, and trajectory and 2) a retrospective thinking stage using a segmentation method to cut the continuous demonstrations into multiple assembly skills optimally. Using MASD, the demonstration of assembly tasks can be explained with high accuracy in real time, driving a hypothesis that a PBD system on the top of MASD can be extended to more realistic assembly tasks beyond pure positional moving and picking. In experiments, the skill identification module is used to recognize the five kinds of assembly skills in demonstrations of both single and multiple assembly skills, and outperforms the comparative action identification methods. Besides integrated with the MASD, the PBD system can generate the program based on the demonstration and successfully enable an ABB industrial robotic arm simulator to assemble a flashlight and a switch, verifying the initial hypothesis.},
  Doi                      = {10.1109/TASE.2017.2783342},
  File                     = {:home/scherzin/Documents/Phd/Literature/Articles/MASD_A_Multimodal_Assembly_Skill_Decoding_System_for_Robot_Programming_by_Demonstration.pdf:PDF},
  ISSN                     = {1545-5955},
  Keywords                 = {Decoding;Education;Programming;Real-time systems;Service robots;Activity recognition;robot learning;robot programming.}
}

@Article{Zhou2014,
  Title                    = {Is Joint Training Better for Deep Auto-Encoders?},
  Author                   = {Zhou, Yingbo and Arpit, Devansh and Nwogu, Ifeoma and Govindaraju, Venu},
  Journal                  = {arXiv preprint arXiv:1405.1380},
  Year                     = {2014},

  File                     = {:home/scherzin/Documents/Phd/Literature/Papers/Is_Joint_Training_Better_for_Deep_Auto-Encoders.pdf:PDF},
  Url                      = {https://arxiv.org/abs/1405.1380}
}

@Comment{jabref-meta: databaseType:bibtex;}

@Comment{jabref-meta: grouping:
0 AllEntriesGroup:;
1 StaticGroup:Markings\;2\;1\;\;\;\;;
2 StaticGroup:scherzin:1\;2\;1\;\;\;\;;
2 StaticGroup:scherzin:2\;2\;1\;\;\;\;;
}

